Nussbaum Function Based Approach for Tracking Control of Robot Manipulators

This paper introduces a novel Nussbaum function-based PID control for robotic manipulators. The integration of the Nussbaum function into the PID framework provides a solution with a simple structure that effectively tackles the challenge of unknown control directions. Stability is achieved through a combination of neural network-based estimation and Lyapunov analysis, facilitating automatic gain adjustment without the need for system dynamics. Our approach offers a gain determination with minimum parameter requirements, significantly reducing the complexity and enhancing the efficiency of robotic manipulator control. The paper guarantees that all signals within the closed-loop system remain bounded. Lastly, numerical simulations validate the theoretical framework, confirming the effectiveness of the proposed control strategy in enhancing robotic manipulator control.

==> Aircraft/00-Abstract.tex <==
\begin{abstract}


Nussbaum Gain Adaptive Neural Control for Optimized Aircraft spin Recovery Maneuvers.

\end{abstract}

==> Aircraft/01-Intro.tex <==
\section{Introduction}
\label{sec_intro}

==> Aircraft/02-Dynamic.tex <==
\section{Dynamics Formulation}
\label{sec_Dyn}

==> Aircraft/03-Control.tex <==
\section{Control Design}
\label{sec_control}
\noindent Dynamics

\begin{equation} \label{1)} 
M\ddot{q}+C\dot{q}+G=\kappa \tau + f_h 
\end{equation} 

Define 

\begin{equation} \label{2)} 
\Xi =2k_{0} e+k_{0}^{2} \int e +\dot{e} 
\end{equation} 

And choose

\begin{equation} \label{3)} 
\tau =K_{D} \Xi  
\end{equation} 

Where $K_{D} =k_{d} +\kappa _{D} ,$ and  $k_{d} =Nk_{\Delta } $ with $k_{\Delta } $ is a positive constant, and $\kappa _{D} =N\kappa _{\Delta } $ with $\kappa _{\Delta } =\alpha \hat{\omega }^{T} h$ with the adaptive law as,

\begin{equation} \label{6)} 
\dot{\hat{\omega }}=\Gamma \left(\alpha \left\| \Xi \right\| ^{2} h-\sigma \hat{\omega }\right) 
\end{equation} 

We selected Nussbaum type function as $N=\zeta^2\cos{\zeta}$, where $\zeta$ is updated by 
\begin{equation} \label{2)} 
\dot{\zeta }=\Xi ^{T} \left(k_{\Delta } +\kappa _{\Delta } \right)\Xi .
\end{equation}

Consider 

\begin{equation} \label{5)} 
V=\frac{1}{2} \Xi ^{T} M\Xi +\frac{1}{2} \tilde{\omega }^{T} \Gamma ^{-1} \tilde{\omega } 
\end{equation} 

Then, considering robot dynamics properties @, and by using RBF NN to approximate uncertainties, we have $f_{uncertain} =\omega ^{*^{T} } h+\varpi $where $\varpi \le \varpi _{M} $, then

% \begin{equation} \label{9)} 
% \dot{V}\le \kappa N\dot{\zeta }+\dot{\zeta }-\Xi ^{T} k_{\Delta } \Xi +\Xi ^{T} \varpi +\sigma \tilde{\omega }^{T} \hat{\omega }. 
% \end{equation} 




==> Aircraft/04-Simulation.tex <==
\section{Illustrative examples}
\label{sec_simulation}

==> Aircraft/05-Experiment.tex <==
\section{Experimental Results}
\label{sec_experiment}

==> Aircraft/06-Disussion.tex <==
\section{Discussion}
\label{sec_discussion}

==> Aircraft/07-Conclusion.tex <==
\section{Conclusion}
\label{sec_conclusion}


In this paper,

==> Robot/06-Discuss.tex <==
\section{Discussion}
\label{sec_discussion}


\paragraph{Removing $k_d$}


\paragraph{Automatic $\alpha$}

==> Robot/To_be_added.tex <==
\section{To be added}
\label{sec_conclusion}

Consider the accumulated error function \(\Xi\) defined as 
\begin{equation}
\Xi(t) = 2{\upsilon}e(t) + {\upsilon}^2\int_0^t e(t) \,d\rho + \frac{de(t)}{dt},
\end{equation}
where \(e(t)\) is the error function, representing the difference between the desired trajectory and the actual trajectory in a control system.

Let \(\upsilon\) be given by
\begin{equation}
{\upsilon}=W_c^Th,
\end{equation}
where \(W_c\) represents the weight matrix of the critic network and \(h\) is a vector of basis functions.

To minimize the error \(\Xi\), the objective function \(E_c\) is defined as 
\begin{equation} \label{eq_ObjF}
E_c = \frac{1}{2}{\Xi^T}\Xi,
\end{equation}
which represents the half of the squared norm of \(\Xi(t)\). The minimization of \(E_c\) aims to reduce the squared error, a common objective in control and optimization problems.

The updating law for the critic network, based on the gradient descent method, is derived as follows:
\begin{equation} \label{eq_wdotc 1}
{\dot {\hat {W}}_c} =  - {\sigma}\frac{{\partial {E_c}}}{{\partial {{\hat W}_c}}} = - {\sigma}\frac{\partial{E_c}}{\partial{\Xi}}\frac{\partial{\Xi}}{\partial{\upsilon}}\frac{\partial{\upsilon}}{\partial{W_c}},
\end{equation}
where \(\sigma > 0\) is the learning rate.

Calculating each term in Equation \ref{eq_wdotc 1}, we have:
\begin{align*}
\frac{\partial E_c}{\partial \Xi} &= \Xi, \\
\frac{\partial \Xi}{\partial \upsilon} &= 2e(t) + 2\upsilon\int_0^t e(t) \,d\rho, \\
\frac{\partial \upsilon}{\partial W_c} &= h.
\end{align*}

Substituting these into Equation \ref{eq_wdotc 1}, we get:
\begin{equation}
{\dot {\hat {W}}_c} = -2\sigma \Xi \left(e(t) + \upsilon\int_0^t e(t) \,d\rho\right) h.
\end{equation}


==> name.tex <==


\begin {figure}[h]%[!hbtp]
 \centering
  \begin{adjustbox}{width=\textwidth*19/40}
%  \includegraphics[width=8.5cm]




\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da28347712058597496] 
\draw    (8.73,152.32) -- (88.16,152.5) ;
\draw [shift={(90.16,152.5)}, rotate = 180.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp9311221548800159] 
\draw   (91,130) -- (183,130) -- (183,175) -- (91,175) -- cycle ;
%Straight Lines [id:da47922216302447707] 
\draw    (182.73,152.32) -- (276.55,152.5) ;
\draw [shift={(278.55,152.5)}, rotate = 180.11] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp213972983459354] 
\draw   (278,133) -- (373.55,133) -- (373.55,172) -- (278,172) -- cycle ;
%Straight Lines [id:da35736119238888575] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (322.73,88.32) -- (322.03,130) ;
\draw [shift={(322,132)}, rotate = 270.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Straight Lines [id:da14706676861609203] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (373.36,152.5) -- (482.36,152.5) ;
\draw [shift={(484.36,152.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% Text Node
\draw (138,152.5) node   [align=left] {\begin{minipage}[lt]{53.16pt}\setlength\topsep{0pt}
\begin{center}
Pose
\end{center}
 Estimation
\end{minipage}};
% Text Node
\draw (285,144) node [anchor=north west][inner sep=0.75pt]   [align=left] {LfD/Planning};
% Text Node
\draw (5,126) node [anchor=north west][inner sep=0.75pt]   [align=left] {Object Model};
% Text Node
\draw (188,126) node [anchor=north west][inner sep=0.75pt]   [align=left] {Grasping Point};
% Text Node
\draw (247,71) node [anchor=north west][inner sep=0.75pt]   [align=left] {Human Demonstration};
% Text Node
\draw (378,128) node [anchor=north west][inner sep=0.75pt]   [align=left] {Robot Assembly};


\end{tikzpicture}



  \end{adjustbox}
	\caption{The overview of the automated industrial manipulation pipeline.}\label{FIG_Overall}
\end{figure}
